AIMY: An Open-source Table Tennis Ball Launcher for Versatile and High-fidelity Trajectory Generation

To approach the level of advanced human players in table tennis with robots, generating varied ball trajectories in a reproducible and controlled manner is essential. Current ball launchers used in robot table tennis either do not provide an interface for automatic control or are limited in their capabilities to adapt speed, direction, and spin of the ball. For these reasons, we present AIMY, a three-wheeled open-hardware and open-source table tennis ball launcher, which can generate ball speeds and spins of up to 15.4 ms-1 and 192 s-1, respectively, which are comparable to advanced human players. The wheel speeds, launch orientation and time can be fully controlled via an open Ethernet or Wi-Fi interface. We provide a detailed overview of the core design features, as well as open source the software to encourage distribution and duplication within and beyond the robot table tennis research community. We also extensively evaluate the ball launcher's accuracy for different system settings and learn to launch a ball to desired locations. With this ball launcher, we enable long-duration training of robot table tennis approaches where the complexity of the ball trajectory can be automatically adjusted, enabling large-scale real-world online reinforcement learning for table tennis robots.

==> archive/99_archive.tex <==
\newpage
\section*{APPENDIX}

\textbf{Technical specifications:}
Altitude Angle: approx. \ang{49} - \ang{81} \\
Azimuthal Angle: approx. $\pm$\ang{23} \\
Supply: 230V (50~Hz)

\textbf{Abbreviations:}
ITTF - International Table Tennis Federation
ESC - Electronic Speed Control
GPIO - General-Purpose Input/Output
API - Application Programming Interface
RL - Reinforcement Learning
3D - three dimensional
MLP - Multilayer Perceptron
TCP - Transmission Control Protocol
AIMY - diminutive of the word aimbot, female name


\textbf{Third Party Hardware:}
Launch motor - T-MOTOR Antigravity MN4004 KV300
Launch motor - T-MOTOR Antigravity MN5008 KV170
ESC - T-MOTOR AIR 40A
Azimuthal servomotor launch unit - Hitec D954SW
Altitude linear actuator - Actuoinx L12-30-210-6-R

Reservoir Stirrer - Pololu SpringRC SM-S4303R
Ball Feeding Unit - Hitec HSB-9381TH 

Central Control Unit - Raspberry Pi 4 Model B
Interface - Raspberry Pi Touch Display (7 inch)

Launch motor driver - Xinabox OC05
Launch motor throw wheel - AMICUS Ball Throw Wheel
Launch unit azimuthal bearing - Franke LEL1\_5\_0070

Power Supply Unit - Mean Well HDR-150-24 (24 V)
Power Supply Unit - Mean Well MDR-40-5 (5 V)

\input{tables/rampup}
\input{tables/jump}
\input{tables/strokegain}
\input{tables/pinching}


For better evaluation on the design objectives of a custom designed ball launcher, further knowledge of human capabilities in terms of ball speed and spin generation is necessary. Wu et al. measured ball spins up to $151.3 \frac{1}{s}$ revolutions per second during matches with players from the Chinese National Team and the Youth Chinese National Team of 1987 \cite{wu1992}. After changes of the International Table Tennis Federation of the official table tennis ball with an increased diameter and a switch from celluloid material to plastic Lee et al. \cite{lee2019} evaluated maximum speeds up to $20.16 \frac{m}{s}$ and ball spins up to $ 132.3 \frac{1}{s}$ among players on national table-tennis team and youth national table-tennis team level. The magnitude of these values are roughly confirmed by \cite{xie2002, blank2017}.

In the following, we provide an overview of the core design features and components, along with the corresponding low-level control software. Subsequently, the repetition accuracy is evaluated for different system parameters like stroke speed for the ball feeding system, the ball pinch in the launch unit, orientation jumps of the launching unit and the ramp-up time of the motors until launch. Furthermore, AIMY is validated for different launching distances compared to a commercially available product. Beside the supplementary materials for distribution and duplication of AIMY, this publication also provides a feed-forward based control approach for target shooting as well as a rich data set of more than 3.761 recorded and filtered ball trajectories.

\subsubsection{Orientation jumps in the launch unit}
For high fidelity, the orientation of the launch unit should be as similar as possible for the similar parameters. Therefore, it was investigated whether there is an increased deviation of landing points after a realignment to the same orientation. For this, on one side trajectories were recorded without orientation change and on the other side, after each launch, the launch unit was moved to the lowest altitude angle and the leftmost azimuthal angle. Before the launch, the launch unit was then moved back to its initial position. The result of this experiment can be seen in Table~\ref{tab:jump}.

No significant deviation due to jumps in orientation could be detected on the basis of the measurement data.

\subsubsection{Ramp-up time of the motors}
Basically, two operating modes of the motors are possible depending on the usage. For example, in the case of long intervals between each launch, the motors can be stopped after launch and started up again shortly before the next launch. The other operation mode is continuous rotation of the wheels enabling steady and gentle operation of the motors. The resulting standard deviations of the landing points for different ramp-up times is shown in Table~\ref{tab:rampup} and illustrated in Figure.

Based on the results from the evaluation, it can be shown that ramp-up times lower than 0.5 seconds produce an increased deviation. This can be explained by the fact that a stationary speed has not yet been reached until launch. A ramp-up time of 3.0 seconds showed the lowest deviation with respect to the area of deviation in x- and y-direction. However, the differences are not statistically significant. Continuous operation provides similar low deviations and is recommended for long-duration training due to the gentle operation of the motors. 

\subsubsection{Ball pinch in the launch unit}

Ball pinching refers to the maximum compression of the ball by the throwing wheels during the launch procedure. The individual wheel units can be installed on the launch unit with different radial distances to the center. The smaller the distance, the higher the pressure generated on the ball during the launching. In the following, the influence of different pressures on the deviation of the landing position will be investigated. For setup of different pinching cylindrical gauge blocks are used. It can be assumed that pinching smaller than the ball diameter will result in larger deviations, therefore only pinching smaller than the standardised ball diameter is evaluated. The standard deviations of the landing points with different pinching is shown in Table~\ref{tab:pinching}. 

In the measurements, 37.4 mm pinching shows the smallest deviation. Considering statistical deviation, it can be stated that a range between 36.0 and 38.0 mm produces the smallest deviation in landing position. 

\subsubsection{Stroke gain of the ball feeding system}

The stroke gain influences the speed at which the balls are fed to the launch unit. With each control loop pass, the stroke gain increases with the stroke position and allows steady insertion of the table tennis balls. The effect of the stroke speed is illustrated in Subsection~\ref{sub:hardware} in Figure~\ref{fig:feeding_system}. Based on the measurement data, shown in Table~\ref{tab:strokegain}, no significant influence of the stroke speed on the position accuracy can be shown for stroke gains above 0.50. While 0.05 and 0.10 show noteworthy decreased standard deviations, they result in increased launching times, which can be disadvantageous for long-duration experiments as common with RL.

\begin{table}[H]
\centering
\caption{}
\label{tab:dataset}
\begin{tabular}{@{}ccl@{}}
\toprule
\# & \begin{tabular}[c]{@{}c@{}}Number\\ samples\end{tabular} & \multicolumn{1}{c}{Description} \\ \midrule
1 & 415 & \begin{tabular}[c]{@{}l@{}}Launching only similar launch speeds \\ of all wheels. No or low initial spin.\end{tabular} \\ \midrule
2 & 64 & \begin{tabular}[c]{@{}l@{}}Launching only with large wheel speed \\ deviations. Trajectories with large spin.\end{tabular} \\ \midrule
3 & 364 & \begin{tabular}[c]{@{}l@{}}Launching only with low wheel speeds.\\ Trajectories with low to medium spin.\end{tabular} \\ \midrule
4 & 1103 & \begin{tabular}[c]{@{}l@{}}Launching only with high altitude \\ angles. Low to large spin is possible.\end{tabular} \\ \midrule
5 & 1385 & \begin{tabular}[c]{@{}l@{}}Launching only with medium altitude \\ angles. Low to medium spin is possible.\end{tabular} \\ \midrule
6 & 430 & \begin{tabular}[c]{@{}l@{}}Launching only with low altitude angles.\\ Low spin is possible.\end{tabular} \\ \midrule
Total & 3761 &  \\ \bottomrule
\end{tabular}
\end{table}

==> archive/graphics/rampup_plot.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{black34}{RGB}{34,34,34}
\definecolor{gray}{RGB}{128,128,128}
\definecolor{indianred20783105}{RGB}{207,83,105}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{teal0108102}{RGB}{1,147,215}
\definecolor{whitesmoke}{RGB}{245,245,245}

\begin{axis}[
axis background/.style={fill=whitesmoke},
axis line style={gray},
height=4.0cm,
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204, fill=whitesmoke},
tick align=outside,
width=8.0cm,
x grid style={white},
xlabel=\textcolor{black34}{\(\displaystyle t_{ramp}\) [s]},
xmajorgrids,
xmajorticks=false,
xmin=-0.5, xmax=12,
xtick style={color=black34},
y grid style={white},
ylabel=\textcolor{black34}{\(\displaystyle \sigma\) [m]},
ymajorgrids,
ymajorticks=false,
ymin=0.0118378456058421, ymax=0.0451120730937024,
ytick style={color=black34}
]
\addplot [line width=0.48pt, indianred20783105, mark=*, mark size=2.4, mark options={solid}]
table {%
0.01 0.0401689226222973
0.05 0.0400360561215795
0.1 0.0435996082078906
0.5 0.0211268140636482
1 0.0242869301473277
2 0.0243445778226545
3 0.0234409623199056
8 0.0237327250540187
15 0.0231068482921517
};
\addlegendentry{$\sigma_x$}
\addplot [line width=0.48pt, teal0108102, mark=*, mark size=2.4, mark options={solid}]
table {%
0.01 0.0165665564742826
0.05 0.0143320032042472
0.1 0.0174283277285046
0.5 0.0150007166933308
1 0.0171740209751143
2 0.0134113465678336
3 0.0133503104916539
8 0.0172763155274512
15 0.0150455328140189
};
\addlegendentry{$\sigma_y$}
\end{axis}

\end{tikzpicture}

